A mixed formulation for physics-informed neural networks as a potential solver for engineering problems in heterogeneous domains: comparison with finite element method

Physics-informed neural networks (PINNs) are capable of finding the solution for a given boundary value problem. We employ several ideas from the finite element method (FEM) to enhance the performance of existing PINNs in engineering problems. The main contribution of the current work is to promote using the spatial gradient of the primary variable as an output from separated neural networks. Later on, the strong form which has a higher order of derivatives is applied to the spatial gradients of the primary variable as the physical constraint. In addition, the so-called energy form of the problem is applied to the primary variable as an additional constraint for training. The proposed approach only required up to first-order derivatives to construct the physical loss functions. We discuss why this point is beneficial through various comparisons between different models. The mixed formulation-based PINNs and FE methods share some similarities. While the former minimizes the PDE and its energy form at given collocation points utilizing a complex nonlinear interpolation through a neural network, the latter does the same at element nodes with the help of shape functions. We focus on heterogeneous solids to show the capability of deep learning for predicting the solution in a complex environment under different boundary conditions. The performance of the proposed PINN model is checked against the solution from FEM on two prototype problems: elasticity and the Poisson equation (steady-state diffusion problem). We concluded that by properly designing the network architecture in PINN, the deep learning model has the potential to solve the unknowns in a heterogeneous domain without any available initial data from other sources. Finally, discussions are provided on the combination of PINN and FEM for a fast and accurate design of composite materials in future developments.

==> bib.tex <==
%% paper PINNs AH 
@article{Blechschmidt2021,
  title={Three ways to solve partial differential equations with neural networks — A review},
  author={Jan Blechschmidt and Oliver G. Ernst},
  journal={GAMM‐Mitteilungen},
  year={2021},
  volume={44}
}


% Old papers
@article{Psichogios1992,
author = {Psichogios, Dimitris C. and Ungar, Lyle H.},
title = {A hybrid neural network-first principles approach to process modeling},
journal = {AIChE Journal},
volume = {38},
number = {10},
pages = {1499-1511},
year = {1992}
}

@article{LEE1990,
title = {Neural algorithm for solving differential equations},
journal = {Journal of Computational Physics},
volume = {91},
number = {1},
pages = {110-131},
year = {1990},
issn = {0021-9991},
author = {Hyuk Lee and In Seok Kang},
}


@ARTICLE{Lagaris1998,
  author={Lagaris, I.E. and Likas, A. and Fotiadis, D.I.},
  journal={IEEE Transactions on Neural Networks}, 
  title={Artificial neural networks for solving ordinary and partial differential equations}, 
  year={1998},
  volume={9},
  number={5},
  pages={987-1000},
  }
  
  
@article{Kondor2018,
author = {Kondor, Risi and Trivedi, Shubhendu},
year = {2018},
title = {On the Generalization of Equivariance and Convolution in Neural Networks to the Action of Compact Groups}
}


@article{Guo2022,
author = {Guo, Hongwei and Zhuang, Xiaoying and Chen, Pengwan and Alajlan, Naif and Rabczuk, Timon},
year = {2022},
journal={Engineering with Computers}, 
title = {Analysis of three-dimensional potential problems in non-homogeneous media with physics-informed deep collocation method using material transfer learning and sensitivity analysis}
}


@article{GOSWAMI2022114587,
title = {A physics-informed variational DeepONet for predicting crack path in quasi-brittle materials},
journal = {Computer Methods in Applied Mechanics and Engineering},
volume = {391},
pages = {114587},
year = {2022},
author = {Somdatta Goswami and Minglang Yin and Yue Yu and George Em Karniadakis},
}


%% Raissi 
@article{RAISSI2019,
title = {Physics-informed neural networks: A deep learning framework for solving forward and inverse problems involving nonlinear partial differential equations},
journal = {Journal of Computational Physics},
volume = {378},
pages = {686-707},
year = {2019},
author = {M. Raissi and P. Perdikaris and G.E. Karniadakis},
}

@article{RAISSI2018,
title = {Hidden physics models: Machine learning of nonlinear partial differential equations},
journal = {Journal of Computational Physics},
volume = {357},
pages = {125-141},
year = {2018},
author = {Maziar Raissi and George Em Karniadakis},
}



@article{Raissi2020fluidflow,
author = {Maziar Raissi  and Alireza Yazdani  and George Em Karniadakis },
title = {Hidden fluid mechanics: Learning velocity and pressure fields from flow visualizations},
journal = {Science},
volume = {367},
number = {6481},
pages = {1026-1030},
year = {2020},
}


@article{Raissi2019Vortex, 
title={Deep learning of vortex-induced vibrations}, 
journal={Journal of Fluid Mechanics}, 
publisher={Cambridge University Press}, 
author={Raissi, Maziar and Wang, Zhicheng and Triantafyllou, Michael S. and Karniadakis, George Em}, 
year={2019}, 
pages={119–137}
}


@article{Raissi2019Turbulance,
  title = {Deep learning of turbulent scalar mixing},
  author = {Raissi, Maziar and Babaee, Hessam and Givi, Peyman},
  journal = {Phys. Rev. Fluids},
  volume = {4},
  issue = {12},
  pages = {124501},
  numpages = {14},
  year = {2019},
  publisher = {American Physical Society},
}


@article{JAGTAP2020,
title = {Conservative physics-informed neural networks on discrete domains for conservation laws: Applications to forward and inverse problems},
journal = {Computer Methods in Applied Mechanics and Engineering},
volume = {365},
pages = {113028},
year = {2020},
author = {Ameya D. Jagtap and Ehsan Kharazmi and George Em Karniadakis},
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Haghighat va bad az an
@article{HAGHIGHAT2021,
title = {A physics-informed deep learning framework for inversion and surrogate modeling in solid mechanics},
journal = {Computer Methods in Applied Mechanics and Engineering},
volume = {379},
pages = {113741},
year = {2021},
author = {Ehsan Haghighat and Maziar Raissi and Adrian Moure and Hector Gomez and Ruben Juanes},
}


%% becha paderborn
@article{Henkes2022,
author = {Henkes, Alexander and Wessels, Henning and Mahnken, Rolf},
title = {Physics informed neural networks for continuum micromechanics},
journal = {PAMM},
volume = {21},
number = {1},
pages = {e202100040},
abstract = {Abstract The present work proposes a Physics Informed Neural Network (PINN) for solving boundary value problems in continuum micromechanics. The presented technique is therefore an alternative to the finite element method or Fourier transform based methods. In this context, a neural network is used to approximate the function solving the partial differential equation. The theory of PINN in the context of micromechanics is developed.},
year = {2021}
}


% Multi Physics 
@incollection{Nguyen2022,
  title={Efficient Physics Informed Neural Networks Coupled with Domain Decomposition Methods for Solving Coupled Multi-physics Problems},
  author={Nguyen, Long and Raissi, Maziar and Seshaiyer, Padmanabhan},
  booktitle={Advances in Computational Modeling and Simulation},
  pages={41--53},
  year={2022},
  publisher={Springer}
}


@article{He2020,
author = {He, Qizhi and Barajas-Solano, David and Tartakovsky, Guzel and Tartakovsky, Alexandre},
year = {2020},
month = {05},
pages = {103610},
title = {Physics-Informed Neural Networks for Multiphysics Data Assimilation with Application to Subsurface Transport},
volume = {141},
journal = {Advances in Water Resources},
}

@article{PATEL2022,
title = {Thermodynamically consistent physics-informed neural networks for hyperbolic systems},
journal = {Journal of Computational Physics},
volume = {449},
pages = {110754},
year = {2022},
author = {Ravi G. Patel and Indu Manickam and Nathaniel A. Trask and Mitchell A. Wood and Myoungkyu Lee and Ignacio Tomas and Eric C. Cyr},
}

@article{GOSWAMI2020,
title = {Transfer learning enhanced physics informed neural network for phase-field modeling of fracture},
journal = {Theoretical and Applied Fracture Mechanics},
volume = {106},
pages = {102447},
year = {2020},
author = {Somdatta Goswami and Cosmin Anitescu and Souvik Chakraborty and Timon Rabczuk},
}


%% SciANN
@article{SciANN,
title = {SciANN: A Keras/TensorFlow wrapper for scientific computations and physics-informed deep learning using artificial neural networks},
journal = {Computer Methods in Applied Mechanics and Engineering},
volume = {373},
pages = {113552},
year = {2021},
author = {Ehsan Haghighat and Ruben Juanes},
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{Bock2019,
AUTHOR={Bock, Frederic E. and Aydin, Roland C. and Cyron, Christian J. and Huber, Norbert and Kalidindi, Surya R. and Klusemann, Benjamin},   
TITLE={A Review of the Application of Machine Learning and Data Mining Approaches in Continuum Materials Mechanics},      
JOURNAL={Frontiers in Materials},      
VOLUME={6},      
YEAR={2019},      
}


@article{Cai2022,
title = {Physics-informed neural networks (PINNs) for fluid mechanics: a review},
journal = {Acta Mechanica Sinica},
year = {2022},
author = {Cai, Shengze and Mao, Zhiping and Wang, Zhicheng and Yin, Minglang and Karniadakis, George Em},
}


@article{Rao2021,
author = {Chengping Rao  and Hao Sun  and Yang Liu },
title = {Physics-Informed Deep Learning for Computational Elastodynamics without Labeled Data},
journal = {Journal of Engineering Mechanics},
volume = {147},
number = {8},
pages = {04021043},
year = {2021},
}


@misc{Bhaduri2021,
  author = {Bhaduri, Anindya and Gupta, Ashwini and Graham-Brady, Lori},
  title = {Stress field prediction in fiber-reinforced composite materials using a deep learning approach},
  publisher = {arXiv},
  year = {2021},
  copyright = {arXiv.org perpetual, non-exclusive license}
}



@misc{Minglang2022,
  author = {Yin, Minglang and Zhang, Enrui and Yu, Yue and Karniadakis, George Em},
  title = {Interfacing Finite Elements with Deep Neural Operators for Fast Multiscale Modeling of Mechanics Problems},
  publisher = {arXiv},
  year = {2022},
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{mianroodi2021teaching,
  title={Teaching solid mechanics to artificial intelligence—a fast solver for heterogeneous materials},
  author={Mianroodi, Jaber Rezaei and H Siboni, Nima and Raabe, Dierk},
  journal={npj Computational Materials},
  volume={7},
  number={1},
  pages={1--10},
  year={2021},
  publisher={Nature Publishing Group}
}

@misc{Yin2022,
  author = {Yin, Minglang and Zhang, Enrui and Yu, Yue and Karniadakis, George Em},
  title = {Interfacing Finite Elements with Deep Neural Operators for Fast Multiscale Modeling of Mechanics Problems},
  publisher = {arXiv},
  year = {2022},
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@article{mianroodi2022lossless,
  title={Lossless multi-scale constitutive elastic relations with artificial intelligence},
  author={Mianroodi, Jaber Rezaei and Rezaei, Shahed and Siboni, Nima H and Xu, Bai-Xiang and Raabe, Dierk},
  journal={npj Computational Materials},
  volume={8},
  number={1},
  pages={1--12},
  year={2022},
  publisher={Nature Publishing Group}
}

@article{fernandez2020,
  title={Application of artificial neural networks for the prediction of interface mechanics: a study on grain boundary constitutive behavior},
  author={Fern{\'a}ndez, Mauricio and Rezaei, Shahed and Mianroodi, Jaber Rezaei and Fritzen, Felix and Reese, Stefanie},
  journal={Advanced Modeling and Simulation in Engineering Sciences},
  volume={7},
  number={1},
  pages={1--27},
  year={2020},
  publisher={SpringerOpen}
}


@misc{Amini2022,
  author = {Amini, Danial and Haghighat, Ehsan and Juanes, Ruben},
  title = {Physics-informed neural network solution of thermo-hydro-mechanical (THM) processes in porous media},
  publisher = {arXiv},
  year = {2022},
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{Abueidda2022,
  author = {Abueidda, Diab W. and Koric, Seid and Al-Rub, Rashid Abu and Parrott, Corey M. and James, Kai A. and Sobh, Nahil A.},
  title = {A deep learning energy method for hyperelasticity and viscoelasticity},
  publisher = {arXiv},
  year = {2022},
  copyright = {Creative Commons Attribution 4.0 International}
}


@article{BERG201828,
title = {A unified deep artificial neural network approach to partial differential equations in complex geometries},
journal = {Neurocomputing},
volume = {317},
pages = {28-41},
year = {2018},
author = {Jens Berg and Kaj Nyström},
}



@article{Yadav,
author = {Yadav, Gaurav Kumar and Natarajan, Sundararajan and Srinivasan, Balaji},
title = {Distributed PINN for Linear Elasticity — A Unified Approach for Smooth, Singular, Compressible and Incompressible Media},
journal = {International Journal of Computational Methods},
volume = {0},
number = {0},
pages = {2142008},
year = {0},
}


@article{
Zhang2022,
author = {Enrui Zhang  and Ming Dao  and George Em Karniadakis  and Subra Suresh },
title = {Analyses of internal structures and defects in materials using physics-informed neural networks},
journal = {Science Advances},
volume = {8},
number = {7},
pages = {eabk0644},
year = {2022},
}


@misc{Guo2020,
  author = {Guo, Mengwu and Haghighat, Ehsan},
  
  keywords = {Numerical Analysis (math.NA), Machine Learning (cs.LG), FOS: Mathematics, FOS: Mathematics, FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {An energy-based error bound of physics-informed neural network solutions in elasticity},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{Arora2021,
  author = {Arora, Rajat},
  
  keywords = {Machine Learning (cs.LG), Materials Science (cond-mat.mtrl-sci), FOS: Computer and information sciences, FOS: Computer and information sciences, FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Machine Learning-Accelerated Computational Solid Mechanics: Application to Linear Elasticity},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution 4.0 International}
}


@article{SAMANIEGO2020112790,
title = {An energy approach to the solution of partial differential equations in computational mechanics via machine learning: Concepts, implementation and applications},
journal = {Computer Methods in Applied Mechanics and Engineering},
volume = {362},
pages = {112790},
year = {2020},
author = {E. Samaniego and C. Anitescu and S. Goswami and V.M. Nguyen-Thanh and H. Guo and K. Hamdia and X. Zhuang and T. Rabczuk},
}

@article{ZHANG2021100220,
title = {Physics-informed deep learning for digital materials},
journal = {Theoretical and Applied Mechanics Letters},
volume = {11},
number = {1},
pages = {100220},
year = {2021},
author = {Zhizhou Zhang and Grace X Gu},
}


@article{HSU2020197,
title = {Using Deep Learning to Predict Fracture Patterns in Crystalline Solids},
journal = {Matter},
volume = {3},
number = {1},
pages = {197-211},
year = {2020},
author = {Yu-Chuan Hsu and Chi-Hua Yu and Markus J. Buehler},
}


@article{karniadakis2021physics,
  title={Physics-informed machine learning},
  author={Karniadakis, George Em and Kevrekidis, Ioannis G and Lu, Lu and Perdikaris, Paris and Wang, Sifan and Yang, Liu},
  journal={Nature Reviews Physics},
  volume={3},
  number={6},
  pages={422--440},
  year={2021},
  publisher={Nature Publishing Group}
}

@article{Zhang2020PhysicsInformedNN,
  title={Physics-Informed Neural Networks for Nonhomogeneous Material Identification in Elasticity Imaging},
  author={Enrui Zhang and Minglang Yin and George Em Karniadakis},
  journal={ArXiv},
  year={2020},
  volume={abs/2009.04525}
}



@article{Cai2021,
    author = {Cai, Shengze and Wang, Zhicheng and Wang, Sifan and Perdikaris, Paris and Karniadakis, George Em},
    title = "{Physics-Informed Neural Networks for Heat Transfer Problems}",
    journal = {Journal of Heat Transfer},
    volume = {143},
    number = {6},
    year = {2021},
}


@article{JAGTAP2020113028,
title = {Conservative physics-informed neural networks on discrete domains for conservation laws: Applications to forward and inverse problems},
journal = {Computer Methods in Applied Mechanics and Engineering},
volume = {365},
pages = {113028},
year = {2020},
author = {Ameya D. Jagtap and Ehsan Kharazmi and George Em Karniadakis},
}


@article{GOSWAMI2020102447,
title = {Transfer learning enhanced physics informed neural network for phase-field modeling of fracture},
journal = {Theoretical and Applied Fracture Mechanics},
volume = {106},
pages = {102447},
year = {2020},
author = {Somdatta Goswami and Cosmin Anitescu and Souvik Chakraborty and Timon Rabczuk},
}


@article{Bayat2020,
author = {Bayat, Hamid Reza and Rezaei, Shahed and Brepols, Tim and Reese, Stefanie},
title = {Locking-free interface failure modeling by a cohesive discontinuous Galerkin method for matching and nonmatching meshes},
journal = {International Journal for Numerical Methods in Engineering},
volume = {121},
number = {8},
pages = {1762-1790},
year = {2020}
}


@article{LIN2021109193,
title = {Data-driven microstructure sensitivity study of fibrous paper materials},
journal = {Materials \& Design},
volume = {197},
pages = {109193},
year = {2021},
author = {Binbin Lin and Yang Bai and Bai-Xiang Xu},
}

@article{Peng2021,
title = {Multiscale Modeling Meets Machine Learning: What Can We Learn?},
journal = {Archives of Computational Methods in Engineering},
year = {2021},
author = {Peng, Grace C. Y. and Alber, Mark and Buganza Tepole, Adrian and Cannon, William R. and De, Suvranu and Dura-Bernal, Savador and Garikipati, Krishna and Karniadakis, George and Lytton, William W. and Perdikaris, Paris and Petzold, Linda and Kuhl, Ellen},
}

@article{cecen2018material,
  title={Material structure-property linkages using three-dimensional convolutional neural networks},
  author={Cecen, Ahmet and Dai, Hanjun and Yabansu, Yuksel C and Kalidindi, Surya R and Song, Le},
  journal=AM,
  volume={146},
  pages={76--84},
  year={2018},
  publisher={Elsevier}
}

@article{linka2020constitutive,
  title = {Constitutive artificial neural networks: A fast and general approach to predictive data-driven constitutive modeling by deep learning},
journal = {Journal of Computational Physics},
volume = {429},
pages = {110010},
year = {2021},
issn = {0021-9991},
author = {Kevin Linka and Markus Hillgärtner and Kian P. Abdolazizi and Roland C. Aydin and Mikhail Itskov and Christian J. Cyron},
keywords = {Deep learning, Data-driven, Constitutive modeling, Hyperelasticity},
}

@article{MASI2021104277,
title = {Thermodynamics-based Artificial Neural Networks for constitutive modeling},
journal = {Journal of the Mechanics and Physics of Solids},
volume = {147},
pages = {104277},
year = {2021},
issn = {0022-5096},
author = {Filippo Masi and Ioannis Stefanou and Paolo Vannucci and Victor Maffi-Berthier},
}

@article{WANG2018337,
title = {A multiscale multi-permeability poroplasticity model linked by recursive homogenizations and deep learning},
journal = {Computer Methods in Applied Mechanics and Engineering},
volume = {334},
pages = {337-380},
year = {2018},
issn = {0045-7825},
author = {Kun Wang and WaiChing Sun},
}

@article{Kumar2020,
author={Kumar, Siddhant  and Tan, Stephanie and Zheng, Li and Kochmann, Dennis M.},   
title={Inverse-designed spinodoid metamaterials},      
journal={npj Computational Materials},      
volume={6},      
pages={110},     
year={2020},}

@article{Fernandez2021,
title = "Anisotropic hyperelastic constitutive models for finite deformations combining material theory and data-driven approaches with application to cubic lattice metamaterials",
journal = {Computational Mechanics},
volume = "67",
pages = "653–677",
year = "2021",
author = "Fernández, M. and Jamshidian, M. and Böhlke, T. and  Kristian Kersting and Oliver Weeger ",
}


@article {Yangeabd7416,
	author = {Yang, Zhenze and Yu, Chi-Hua and Buehler, Markus J.},
	title = {Deep learning model to predict complex stress and strain fields in hierarchical composites},
	volume = {7},
	number = {15},
	elocation-id = {eabd7416},
	year = {2021},
	publisher = {American Association for the Advancement of Science},
	journal = {Science Advances},
}

@article{ford_machine_2021,
	title = {Machine learning-based accelerated property prediction of two-phase materials using microstructural descriptors and finite element analysis},
	volume = {191},
	journal = CMS,
	author = {Ford, Emily and Maneparambil, Kailasnath and Rajan, Subramaniam and Neithalath, Narayanan},
	month = apr,
	year = {2021},
	pages = {110328},
}

@article{ZOBEIRY2021104232,
title = {A physics-informed machine learning approach for solving heat transfer equation in advanced manufacturing and engineering applications},
journal = {Engineering Applications of Artificial Intelligence},
volume = {101},
pages = {104232},
year = {2021},
author = {Navid Zobeiry and Keith D. Humfeld},
}


%%%%%%%%%%%%%%%%%%%%%
@article{wang2021train,
      title={Train Once and Use Forever: Solving Boundary Value Problems in Unseen Domains with Pre-trained Deep Learning Models}, 
      author={Hengjie Wang and Robert Planas and Aparna Chandramowlishwaran and Ramin Bostanabad},
      year={2021},
      journal={preprint arXiv:2104.10873},
}


@article{Mozaffar2019,
author = {M. Mozaffar  and R. Bostanabad  and W. Chen  and K. Ehmann  and J. Cao  and M. A. Bessa },
title = {Deep learning predicts path-dependent plasticity},
journal = {Proceedings of the National Academy of Sciences},
volume = {116},
number = {52},
pages = {26414-26420},
year = {2019},
}

@article{schmidhuber2015deep,
  title={Deep learning in neural networks: An overview},
  author={Schmidhuber, J{\"u}rgen},
  journal={Neural networks},
  volume={61},
  pages={85--117},
  year={2015},
  publisher={Elsevier}
}


@article{sibi2013analysis,
  title={Analysis of different activation functions using back propagation neural networks},
  author={Sibi, P and Jones, S Allwyn and Siddarth, P},
  journal={Journal of theoretical and applied information technology},
  volume={47},
  number={3},
  pages={1264--1268},
  year={2013}
}


@article{baydin2018automatic,
  title={Automatic differentiation in machine learning: a survey},
  author={Baydin, Atilim Gunes and Pearlmutter, Barak A and Radul, Alexey Andreyevich and Siskind, Jeffrey Mark},
  journal={Journal of Marchine Learning Research},
  volume={18},
  pages={1--43},
  year={2018},
  publisher={Microtome Publishing}
}


@inproceedings{abadi2016tensorflow,
  title={$\{$TensorFlow$\}$: A System for $\{$Large-Scale$\}$ Machine Learning},
  author={Abadi, Mart{\'\i}n and Barham, Paul and Chen, Jianmin and Chen, Zhifeng and Davis, Andy and Dean, Jeffrey and Devin, Matthieu and Ghemawat, Sanjay and Irving, Geoffrey and Isard, Michael and others},
  booktitle={12th USENIX symposium on operating systems design and implementation (OSDI 16)},
  pages={265--283},
  year={2016}
}


@article{paszke2017automatic,
  title={Automatic differentiation in pytorch},
  author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
  year={2017},
  journal={31st Conference on Neural Information Processing Systems },
}


@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}


@article{zeiler2012adadelta,
  title={Adadelta: an adaptive learning rate method},
  author={Zeiler, Matthew D},
  journal={arXiv preprint arXiv:1212.5701},
  year={2012}
}


@inproceedings{ying2019overview,
  title={An overview of overfitting and its solutions},
  author={Ying, Xue},
  booktitle={Journal of Physics: Conference Series},
  volume={1168},
  issue={2},
  pages={022022},
  year={2019},
  organization={IOP Publishing}
}

@article{YU2022114823,
title = {Gradient-enhanced physics-informed neural networks for forward and inverse PDE problems},
journal = {Computer Methods in Applied Mechanics and Engineering},
volume = {393},
pages = {114823},
year = {2022},
author = {Jeremy Yu and Lu Lu and Xuhui Meng and George Em Karniadakis},
}


@misc{Krishna2021,
  author = {Zhang, Xiaoxuan and Garikipati, Krishna},
  
  keywords = {Computational Engineering, Finance, and Science (cs.CE), Machine Learning (cs.LG), Computational Physics (physics.comp-ph), FOS: Computer and information sciences, FOS: Computer and information sciences, FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Bayesian neural networks for weak solution of PDEs with uncertainty quantification},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

